In-Context Learning on a Budget: A Case Study in Token Classification

Few shot in-context learning (ICL) typically assumes access to large annotated training sets. However, in many real world scenarios, such as domain adaptation, there is only a limited budget to annotate a small number of samples, with the goal of maximizing downstream performance. We study various methods for selecting samples to annotate within a predefined budget, focusing on token classification tasks, which are expensive to annotate and are relatively less studied in ICL setups. Across various tasks, models, and datasets, we observe that no method significantly outperforms the others, with most yielding similar results, including random sample selection for annotation. Moreover, we demonstrate that a relatively small annotated sample pool can achieve performance comparable to using the entire training set. We hope that future work adopts our realistic paradigm which takes annotation budget into account.

==> literature_review.tex <==
\subsection{Demonstration Examples Selection}
Extensive research has been conducted on the process of selecting demonstration examples for ICL. One line of research explores the effect of the demonstration examples on the performance of the generative model.
\citet{zhang-etal-2022-active} show that changing the demonstration examples can cause a 30\% increase in performance, while \citet{liu-etal-2022-makes} show that even using the same demonstration examples in a different order might cause a large variance in performance.
\citet{min-etal-2022-rethinking} show that the labels of the demonstration examples can be replaced by random labels with minimal effect to performance, and that the factors that affect performance the most are the label space, the distribution of the demonstration examples text, and the format of the prompt. They did not test on NER.
\citet{li-qiu-2023-finding} show that two examples that boost performance when included separately in the prompt might actually hurt performance when both are added to the prompt.
\citet{an-etal-2023-context} find that the factors that effect the most on the compositional generalization of the generative model are similarity, diversity and complexity of demonstration examples.

A different but related line of research propose different methods for demonstration example selection. Most works assume access to a labeled train set, ignoring the annotation budget.
Some works~\cite{liu-etal-2022-makes, rubin-etal-2022-learning, shi-etal-2022-xricl, li-etal-2023-unified, nan-etal-2023-enhancing} propose to embed the test sample and training samples and use kNN to select demonstration examples.
\citet{zemlyanskiy-etal-2022-generate} first generates a preliminary prediction based on the most similar training samples as demonstrations, and then selects the demonstrations in which the output is most similar to the preliminary prediction.
\citet{li-qiu-2023-finding} first filter the training set to include informative examples only, and then choose a set of demonstration examples that maximize diversity.
\citet{gupta-etal-2023-coverage} propose to select demonstration examples that maximize the informativeness of the entire demonstration set, rather than selecting each demonstration without considering the other selected demonstrations.
\citet{agrawal-etal-2023-context} select demonstration examples by their n-gram overlap with the input, in addition to a single task-level demonstration.
\citet{wu-etal-2023-self} select the list of demonstration examples that minimizes the entropy of the probabilities that the model assigns to the different labels in the label set.
\citet{levy-etal-2023-diverse} propose to select samples that maximize diversity, and show that this improves compositional generalization.
\citet{jiacheng_compositional_2023} explicitly train a retriever for demonstration examples.
\citet{wang2024large} use a small LLM to first learn a latent topic variable and then select demonstrations that maximize the probability of this variable.

Similar to our work, some previous studies identify that in real-word scenarios users don't have access to demonstration pools.
\citet{zhang-etal-2022-active} propose to train a Reinforcement Learning network for selecting demonstration examples from unlabeled data; however, they refrain from creating a pull and instead use the same demonstration examples for all test samples (right?).
Some works \citep{kim2022self, chen-etal-2023-self} prompt the LLM to generate its own demonstration examples.

Most similar to us, \citet{su2022selective} first select an annotated pool from the unlabeled training set, and subsequently select the labeled demonstration examples from this pool. We differ from their study in that we 1) experiment on NER, 2) study multiple pool selection methods, and 3) study the effect of changing the pool size on performance of these different methods.

\subsection{NER}

In the Named Entity Recognition (NER) task, the input is a text, and the output is a list of named entities, each identified by a span of characters in the text and an entity type (e.g., \textbf{person} or \textbf{location}). Previous work has achieved significant success on well-known, publicly available NER datasets~\cite{lample-etal-2016-neural, li-etal-2020-unified}. Recent advances, such as GLiNER \cite{gliner}, have introduced a new variation of the NER task where the desired set of entity types is provided as input to the model.

Since the introduction of in-context learning, several works have examined the use of in-context learning for the NER task.
\citet{chen-etal-2023-learning} propose to train language models as meta functions that can generate new entity extractors.
\citet{zhang2024context} train an demonstration retriever for nested NER using contrastive learning.
Both of these works assume labeled training data, and to the best of our knowledge this work is the first to use in-context learning for NER on a budget.

\subsection{Annotation Budget}

\citet{chang-etal-2021-training} study few-shot learning (fine-tuning on a small set of samples) using a limited annotation budget. They propose to cluster the embeddings of samples in the train set and select one sample from each cluster to be annotated. We study this method as one of our pool selection method (Section~\ref{sec:pool_selection}). Since they study few-shot learning rather than ICL, they select training samples for the entire test set, while we select a pool out of which a small number of demonstration samples will be selected for each test sample.

Mention Retrieval-Augmented Generation (RAG)

==> sections/app_b_sota.tex <==
Table ~\ref{tab:sota} presents the percentage in performance of the best performing model, GPT-4 out of the state-of-the-art, in each dataset:  Ontonotes (92 strict f1-score; ~\citealp{li-etal-2020-dice}) and UNER (86 strict f1-score;~\citealp{mayhew2023universal}).

\input{tables/sota}

==> sections/app_d_additional_results.tex <==
In this section we report additional results on NER using a recently introduced dataset, Universal NER (UNER; \citealp{mayhew2023universal}). The input texts are sourced from the UD dataset. We use the same models, prompts and pool sizes as used for Ontonotes.

\begin{figure*}[tb!]
    \centering
    \includegraphics[width=\textwidth]{figures/uner_results.jpeg}
    \caption{Results for NER using Claude 3 Haiku (left), GPT4 (middle) and Gemini 1.5 Pro (right) on UNER, as a function of the size of sample pool. In methods with a random component we run 3 trials and plot error bars showing the standard deviation. Oracle: using the full training set as the pool.}
    \label{fig:uner_results}
\end{figure*}

Figure~\ref{fig:uner_results} displays the results, reinforcing our conclusions from the main text.

==> tables/dataset_statistics.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{lrr}
\toprule
Dataset & Train  & Test \\
\midrule
Ontonotes & 115,527  & 1,000 \\
UNER & 12,543  & 1,000 \\
\bottomrule
    \end{tabular}
    \caption{Statistics for the datasets used in this study, including the number of train samples and the number of randomly sampled test samples.}
    \label{tab:dataset_statistics}
\end{table}


% \begin{table}[t]
% \centering
% \begin{tabular}{lrrr}
% \toprule
% Dataset & Train & \#Unique & Test \\
% \midrule
% Ontonotes & 115,527 & 4,383 & 1,000 \\
% UNER & 12,543 & 2,938 & 1,000 \\
% \bottomrule
%     \end{tabular}
%     \caption{Statistics for the datasets used in this study, including the number of train samples, the number of unique train samples and the number of randomly sampled test samples.}
%     \label{tab:dataset_statistics}
% \end{table}

==> tables/experiments.tex <==
\begin{table*}[!t]
\centering
\begin{tabular}{ccccccc}
\toprule
 & & 5 & 10 & 20 & 100 & $\infty$ \\
\toprule
\multicolumn{7}{c}{Ontonotes test set} \\
\midrule
\multirow{2}{*}{Random} & strict & 32.98 & 39.70 & 44.37 & 52.13 & 69.99 \\
 & type & 40.28 & 47.08 & 53.24 & 64.90 & 79.23 \\
\multirow{2}{*}{Cluster test} & strict & 34.01 & 37.58 & 40.78 & 54.17 & ???? \\
& type & 40.29 & 44.11 & 51.90 & 64.72 & ???? \\
\multirow{2}{*}{Cluster train} & strict & 32.64 & 38.63 & 42.88 & 57.04 & ???? \\
& type & 39.68 & 48.17 & 51.20 & 70.36 & ???? \\
\multirow{2}{*}{Largest mean} & strict & ???? & ???? & ???? & 54.23 & ???? \\
& type & ???? & ???? & ???? & 65.50 & ???? \\
\midrule
\multicolumn{7}{c}{Yuval's test set} \\
\midrule
\multirow{2}{*}{Random} & strict & ???? & ???? & ???? & ???? & ???? \\
 & type & ???? & ???? & ???? & ???? & ???? \\
\multirow{2}{*}{Cluster test} & strict & ???? & ???? & ???? & ???? & ???? \\
& type & ???? & ???? & ???? & ???? & ???? \\
\multirow{2}{*}{Cluster train} & strict & ???? & ???? & ???? & ???? & ???? \\
& type & ???? & ???? & ???? & ???? & ???? \\
\multirow{2}{*}{Largest mean} & strict & ???? & ???? & ???? & ???? & ???? \\
& type & ???? & ???? & ???? & ???? & ???? \\
\bottomrule
\end{tabular}
\caption{...}
\label{tab:results}
\end{table*}


==> tables/models.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{lrr}
\toprule
Model & \# param & Availability \\
\midrule
Llama-2 & 7B & Open \\
Mistral & 7B & Open \\
Starling & 7B & Open \\
Vicuna & 7B & Open \\
Mixtral & 45B & Open \\
phi-2 & 2.7B & Open \\
GPT-4 & 1760B & Close \\
Claude 3 Haiku & 20B & Close \\
Gemini 1.5 Pro & & \\
\bottomrule
    \end{tabular}
    \caption{...\gabis{I would be more precise regarding the defintion for ``Open'', for example -- Llama is open weights, but not the arechitecure. is this the case for all other ``open'' models?}}
    \label{tab:models}
\end{table}
